bbOCR: An Open-source Multi-domain OCR Pipeline for Bengali Documents

Despite the existence of numerous Optical Character Recognition (OCR) tools, the lack of comprehensive open-source systems hampers the progress of document digitization in various low-resource languages, including Bengali. Low-resource languages, especially those with an alphasyllabary writing system, suffer from the lack of large-scale datasets for various document OCR components such as word-level OCR, document layout extraction, and distortion correction; which are available as individual modules in high-resource languages. In this paper, we introduce Bengali$.$AI-BRACU-OCR (bbOCR): an open-source scalable document OCR system that can reconstruct Bengali documents into a structured searchable digitized format that leverages a novel Bengali text recognition model and two novel synthetic datasets. We present extensive component-level and system-level evaluation: both use a novel diversified evaluation dataset and comprehensive evaluation metrics. Our extensive evaluation suggests that our proposed solution is preferable over the current state-of-the-art Bengali OCR systems. The source codes and datasets are available here: https://bengaliai.github.io/bbocr.

==> table2.tex <==
% \tabcolsep}{7pt}
\begin{table*}[ht]
    \small
    \centering
    \begin{tabular}{|l|ccc|ccc|cc|cc|}  
    
    \Xhline{1\arrayrulewidth}
    	% \textbf{Domain Name} 
     % % &\textbf{NED}$ \downarrow$ 
     % &\textbf{R}$ \uparrow$ &\textbf{P}$ \uparrow$ &\textbf{F1}$ \uparrow$\\  
        \textbf{Metric}& 
        \multicolumn{6}{c|}{\textbf{Word Level }} &
        \multicolumn{4}{c|}{\textbf{Text Level}}
        \\
        \hline
        \textbf{System}& 
        \multicolumn{3}{c|}{\textbf{Tesseract}} &
        \multicolumn{3}{c|}{\textbf{bbOCR}} &
        \multicolumn{2}{c|}{\textbf{Tesseract}} &
        \multicolumn{2}{c|}{\textbf{bbOCR}}
        \\
        \hline
        \textbf{Domain Name} & 
        \textbf{R}$ \uparrow$ & 
        \textbf{P}$ \uparrow$ & 
        \textbf{F}$ \uparrow$ & 
        \textbf{R}$ \uparrow$ & 
        \textbf{P}$ \uparrow$ & 
        \textbf{F}$ \uparrow$ & 
        \textbf{CER}$ \downarrow$ &
        \textbf{WER}$ \downarrow$ & 
        \textbf{CER}$ \downarrow$ &
        \textbf{WER}$ \downarrow$ \\
    \hline\hline
                Book & 0.18 & 0.35 & 0.21 & 0.26 & 0.43 & 0.31 & 0.86 & 1.08 & 0.50 & 0.80 \\ \hline
        Book Cover & 0.15 & 0.60 & 0.21 & 0.33 & 0.87 & 0.41 & 1.06 & 1.15 & 0.68 & 0.75 \\ \hline
        Government Document & 0.12 & 0.26 & 0.16 & 0.25 & 0.48 & 0.31 & 0.94 & 1.05 & 0.91 & 1.02 \\ \hline
        Magazine & 0.22 & 0.50 & 0.26 & 0.41 & 0.63 & 0.47 & 0.80 & 0.94 & 0.80 & 0.97 \\ \hline
        Multi Column Book & 0.27 & 0.54 & 0.32 & 0.42 & 0.62 & 0.47 & 0.85 & 1.03 & 0.64 & 0.83 \\ \hline
        New Newspaper & 0.33 & 0.69 & 0.44 & 0.29 & 0.36 & 0.32 & 0.80 & 0.92 & 0.90 & 1.04 \\ \hline
        Old Newspaper & 0.01 & 0.04 & 0.02 & 0.09 & 0.27 & 0.14 & 0.91 & 1.04 & 1.13 & 1.28 \\ \hline
        Property Document & 0.38 & 0.60 & 0.44 & 0.39 & 0.79 & 0.50 & 0.70 & 0.84 & 0.67 & 0.78 \\ \hline
        Single Column Book & 0.40 & 0.61 & 0.44 & 0.56 & 0.69 & 0.61 & 0.64 & 0.84 & 0.44 & 0.67 \\ \hline
        Per Image Average & 0.28 & 0.50 & 0.32 & 0.41 & 0.60 & 0.46 & 0.78 & 0.97 & 0.59 & 0.80 \\ \hline
    \Xhline{1\arrayrulewidth}
    	
    \end{tabular}
    \\[6pt]
    \caption{System-level performance comparison between bbOCR and Tesseract in different domains in Bengali Language.}
    \label{t1}
% \vspace{-0.25in}
\end{table*}
